LeGend: A Data-Driven Framework for Lemma Generation in Hardware Model Checking

Property checking of RTL designs is a central task in formal verification. Among available engines, IC3/PDR is a widely used backbone whose performance critically depends on inductive generalization, the step that generalizes a concrete counterexample-to-induction (CTI) cube into a lemma. Prior work has explored machine learning to guide this step and achieved encouraging results, yet most methods adopt a per-clause graph analysis paradigm: for each clause they repeatedly build and analyze graphs, incurring heavy overhead and creating a scalability bottleneck. We introduce LeGend, which replaces this paradigm with one-time global representation learning. LeGend pre-trains a domain-adapted self-supervised model to produce latch embeddings that capture global circuit properties. These precomputed embeddings allow a lightweight model to predict high-quality lemmas with negligible overhead, effectively decoupling expensive learning from fast inference. Experiments show LeGend accelerates two state-of-the-art IC3/PDR engines across a diverse set of benchmarks, presenting a promising path to scale up formal verification.

==> tables/specific_cases_comparison_with_deepic3.tex <==

\begin{table*}[t]
  \centering
  \caption{DeepIC3 vs LeGend runtime comparison.}
  \resizebox{\linewidth}{!}{%
\begin{tabular}{lcccccc}
\toprule
\textbf{Benchmark} &
\textbf{DeepIC3--IC3ref} & \textbf{LeGend--IC3ref} & \textbf{Speed-up} &
\textbf{DeepIC3--ABC}    & \textbf{LeGend--ABC}    & \textbf{Speed-up} \\
\midrule\midrule
cal106 & 1578.3 & \best{1077.0} & 1.47 & \best{66.7} & 80.9 & 0.83 \\
qspiflash\_dualflexpress\_divfive-p127 & 1940.3 & \best{1073.5} & 1.81 & 5161.8 & \best{471.6} & 10.95 \\
qspiflash\_dualflexpress\_divfive-p161 & 219.3 & \best{140.5} & 1.56 & 1477.6 & \best{329.8} & 4.48 \\
qspiflash\_dualflexpress\_divthree-p007 & \best{0.7} & 17.3 & 0.04 & 1322.2 & \best{847.7} & 1.56 \\
qspiflash\_dualflexpress\_divthree-p068 & 552.8 & \best{55.4} & 9.99 & 309.4 & \best{207.6} & 1.49 \\
qspiflash\_dualflexpress\_divthree-p094 & 3485.8 & \best{404.2} & 8.62 & \best{198.5} & 553.4 & 0.36 \\
qspiflash\_dualflexpress\_divthree-p106 & \best{508.5} & 676.8 & 0.75 & 564.0 & \best{106.1} & 5.32 \\
qspiflash\_dualflexpress\_divthree-p113 & 1343.2 & \best{182.7} & 7.35 & 313.3 & \best{186.2} & 1.68 \\
qspiflash\_dualflexpress\_divthree-p153 & 1671.2 & \best{141.6} & 11.80 & 7200.0 & 7200.0 & 1.00 \\
qspiflash\_dualflexpress\_divthree-p161 & 604.9 & \best{112.1} & 5.40 & \best{114.3} & 1223.2 & 0.09 \\
qspiflash\_qflexpress\_divfive-p063 & \best{41.0} & 70.0 & 0.58 & 92.1 & \best{56.6} & 1.63 \\
qspiflash\_qflexpress\_divfive-p075 & \best{115.2} & 266.2 & 0.43 & 196.8 & \best{146.9} & 1.34 \\
qspiflash\_qflexpress\_divfive-p107 & \best{9.6} & 45.6 & 0.21 & 72.1 & \best{15.6} & 4.62 \\
zipcpu-busdelay-p46 & \best{7.6} & 12.6 & 0.60 & 64.2 & \best{21.2} & 3.02 \\
\midrule
\textbf{Overall} & 12078.4 & \best{4275.8} & 2.82 & 17153.0 & \best{11446.7} & 1.50 \\
\bottomrule
\end{tabular}
  }%
\end{table*}
